Contact-Implicit Model Predictive Control for Dexterous In-hand Manipulation: A Long-Horizon and Robust Approach

Dexterous in-hand manipulation is an essential skill of production and life. However, the highly stiff and mutable nature of contacts limits real-time contact detection and inference, degrading the performance of model-based methods. Inspired by recent advances in contact-rich locomotion and manipulation, this paper proposes a novel model-based approach to control dexterous in-hand manipulation and overcome the current limitations. The proposed approach has an attractive feature, which allows the robot to robustly perform long-horizon in-hand manipulation without predefined contact sequences or separate planning procedures. Specifically, we design a high-level contact-implicit model predictive controller to generate real-time contact plans executed by the low-level tracking controller. Compared to other model-based methods, such a long-horizon feature enables replanning and robust execution of contact-rich motions to achieve large displacements in-hand manipulation more efficiently; Compared to existing learning-based methods, the proposed approach achieves dexterity and also generalizes to different objects without any pre-training. Detailed simulations and ablation studies demonstrate the efficiency and effectiveness of our method. It runs at 20Hz on the 23-degree-of-freedom, long-horizon, in-hand object rotation task.

==> 1_introduction.tex <==
%
In-hand dexterous manipulation is an essential skill with extensive applications, such as swiveling doorknobs in home service, operating all kinds of tools and machines on the production line and so on.
%
Such a skill is based on contact-rich manipulation, in which the robot needs to make and break contacts to interact with objects \cite{Billard2019TrendsAC}. It is challenging to control the contact-rich motions, because the non-smooth contact mechanism leads to intractable dynamics and stiff loss landscapes \cite{Pang2022GlobalPF}. Although significant efforts have been devoted to the locomotion domain with a great success \cite{Kim2023ContactImplicitMC}, it is quite different with manipulation. For example, the robot needs to actively explore contacts instead of relying on the gravity. Besides, the number and locations of contacts are constantly shifting.
%

%
Existing works adopt both learning-based and model-based approaches to address these challenges. Despite the surprising robustness of learning probably due to domain randomization and large-scale training, its data inefficiency slows down further deployment and generalization \cite{Jin2022TaskDrivenHM, Andrychowicz2018LearningDI, Chen2022VisualDI, Bui2023EnhancingTP, Xu2022AcceleratedPL}.
%

%
In contrast, model-based techniques provide a plug-and-play solution, and can be divided into two categories. The first category, contact-explicit approach, controls the robot to establish contacts around pre-defined locations \cite{Khadivar2023AdaptiveFC}. Thus the manipulation problem turns into the discrete search of contact sequences and the continuous optimization of control inputs \cite{Chen2021TrajectoTreeTO, Cheng2023EnhancingDI, Zhu2022EfficientOM, Cruciani2018DexterousMG}. Although this allows for robust execution on hardware with simple controllers, problems may arise when dealing with long-horizon tasks. Since manipulation with specific contacts easily falls into local optimum, and it is time-consuming to re-plan new sequences.
% problems may arise when generalizing to different systems, since it is time-consuming to obtain new sequences.
The second category adopts a more elegant contact-implicit approach. It is common to use smooth surrogate models \cite{Pang2022GlobalPF, Kurtz2023InverseDT} or relaxed complementary constraints \cite{Kim2023ContactImplicitMC} to enable efficient exploration of possible contacts. The manipulation system is more like a black box with implicitly encoded contacts, thus removing the need for specific contact sequences. However, implicit methods always sacrifice physical fidelity and create difficulties for long-horizon tasks \cite{Kim2023ContactImplicitMC,Pang2022GlobalPF}, since the system is prone to evolving differently under unexpected deviation of contacts.
%

%
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\columnwidth]{figs/introduction/teaser_no_label_v4.pdf}
    \vspace{-10pt}
    \caption{
        %
        \textbf{Overview of the proposed method for long-horizon in-hand manipulation.}
        %
        First, given desired object motions and generalized coordinates, 
        %
        the reference generator infers how to make and break contacts in the system's neighborhood.
        %
        Then, the contact controller remedies modeling errors with tactile feedback and executes the inferred contacts to the fullest.
        %
        Finally, the contact-rich motions are executed with joint-level impedance control.
        %
        The proposed method seamlessly generalizes among different objects.
        %
        % The transparent hand represents previous positions.
        %
    }
    \label{fig: teaser}
    \vspace{-15pt}
\end{figure}
%

%
In this paper, we propose a novel control formulation for long-horizon in-hand manipulation, where the fingers alternately make and break contacts to achieve large displacement of the object, 
% where the contact-rich motions of the multi-finger hand is regulated by cascaded high-level reference generator and low-level contact controller
shown in Fig.~\ref{fig: teaser}. Specifically, the proposed method is realized with a hierarchical structure:
\begin{itemize}
    \item \textbf{At high-level}, we formulate a contact-implicit model predictive control (MPC) scheme to compute reference positions and contact forces given current generalized positions and desired object motions. The controller runs a differential dynamic programming (DDP) algorithm on a smooth, differentiable quasi-dynamic model.
    \item \textbf{At low-level}, we formulate an optimal controller to track the high-level references. The controller incorporates a compliant contact model and reads tactile feedback.
\end{itemize}
%

%
The high-level module infers possible contacts in the system's neighborhood that leads to desired object motions; While the low-level module regulates the system around high-level references to make sure that inferred contacts are executed to the fullest.
% Both modules work in a complementary fashion.
%
Compared to contact-explicit approaches, our method needs no pre-defined trajectories or separate planning procedures. Compared to contact-implicit approaches, our method has superior robustness since it remedies ubiquitous modeling errors. These characteristics enables our method to robustly execute long-horizon manipulation online.
%
In addition, our method works with only trivial warmstart solutions and seamlessly migrates to different objects, without any prior training required in learning-based approaches.
%
Simulation results are presented to demonstrate the better performance of the proposed method compared to existing approaches. Video and codes are available soon on the project website \footnote{https://director-of-g.github.io/in\_hand\_manipulation/}.
%





==> chapters/0_abstract.tex <==
%
Dexterous in-hand manipulation is an essential skill of production and life.
% especially in the emerging trend of general purpose robots.
%
Nevertheless, the highly stiff and mutable features of contacts cause limitations to real-time contact discovery and inference, which degrades the performance of model-based methods.
% which become the stumbling block for model-based methods.
% become the stumbling block for planning and control. Model-based methods has long been hampered by real-time contact discovery and inference,
% leaving the empirical success only to learning-based approaches.
%
Inspired by recent advancements in contact-rich locomotion and manipulation, this paper proposes a novel model-based approach to control dexterous in-hand manipulation and overcome the current limitations.
%
The proposed approach has the attractive feature, which allows the robot to robustly execute long-horizon in-hand manipulation without pre-defined contact sequences or separated planning procedures.
%
Specifically, we design a contact-implicit model predictive controller at high-level to generate real-time contact plans, which are executed by the low-level tracking controller.
%
% Specifically, at high-level, we design a contact-implicit model predictive controller to generate contact sequences with state-of-the-art differentiable contact model; At low-level, we propose an optimal tracking controller with compliant contact model to execute the high-level plans.
%
% Different from existing approaches, the proposed method has superior robustness, due to its real-time performance and the utilization of tactile feedback.
%
Compared with other model-based methods, such a long-horizon feature enables replanning and robust execution of contact-rich motions to achieve large-displacement in-hand tasks more efficiently; Compared with existing learning-based methods, the proposed approach achieves the dexterity and also generalizes to different objects without any pre-training.
% i.e., no predefined contact sequences or separated planning procedure are needed
%
Detailed simulations and ablation studies demonstrate the efficiency and effectiveness of our method. It runs at 20Hz on the 23-degree-of-freedom long-horizon in-hand object rotation task.
%


==> chapters/2_related_work.tex <==
%
Dexterous in-hand manipulation refers to manipulating objects without a place-and-re-grasp process \cite{Cruciani2020BenchmarkingIM}.
%
We discuss existing approaches for in-hand manipulation in this section. Several enlightening works from a more general contact-rich locomotion and manipulation domain are included, while we omit innovations purely in mechanical design.
%

\subsubsection{With Reinforcement-Learning (RL) or Imitation-Learning (IL)}
%
Recently, learning-based approaches have exhibited excellent performance and stability in dexterous in-hand manipulation \cite{Weinberg2024SurveyOL}. RL-based and IL-based methods are the mainstream.
%
The empirical success of RL can be attributed to inner stochasticity \cite{Pang2022GlobalPF}, domain randomization, flexible choice of sensing modalities \cite{Andrychowicz2018LearningDI} and large-scale training with memory \cite{Chen2022VisualDI}.
%
Different from RL, extensive exploration of the action space is less needed for IL. However, IL-based methods rely heavily on expert demonstrations \cite{Qin2022FromOH}.
%
Some other methods use model-driven learning \cite{Kumar2016OptimalCW, Weinberg2024SurveyOL}, or explore the combination with non-learning approaches \cite{Jin2022TaskDrivenHM, Bui2023EnhancingTP, Xu2022AcceleratedPL}.
%
Nevertheless, learning-based methods understand the mechanism of in-hand manipulation mainly from data, thus they struggle to capture the inner commonalities from a theoretic perspective. Therefore, such methods may not perform well for unseen objects or in the presence of significant sim2real gaps.
%

\subsubsection{Model-Based Design Using Explicitly Represented Contacts}
%
Model-based techniques provide a training-free solution to deployment and generalization.
%
For planning and control in dexterous in-hand manipulation, the most common way is to represent contacts explicitly. The contact sequences often contain their locations, modes, reaction forces and so on \cite{Cheng2023EnhancingDI}.
%
Existing works adopt searching \cite{Chen2021TrajectoTreeTO, Zhu2022EfficientOM, Cruciani2018DexterousMG}, sampling \cite{Cheng2023EnhancingDI, Dafle2018InHandMV} or demonstration \cite{Khadivar2023AdaptiveFC} to obtain such discrete sequences.
%
The subsequent procedure is simplified to solving for the continuous control inputs, e.g., joint torques, while following pre-defined contact sequences \cite{Chen2021TrajectoTreeTO}. Thus the low-level control usually transforms into easy-to-solve optimization problems with force closure and non-sliding constraints.
%
Although these methods are easier and more precise to implement on hardware, the additional acquisition of contact sequences adds too much complexity and degrades real-time performance. Moreover, if the contact states deviate from pre-defined ones due to disturbance, the specific contact sequence becomes misleading information.
%


\subsubsection{Model-Based Design Using Implicitly Encoded Contacts}
%
Several works avoid the expanding complexity of explicit contact representation with the help of (relaxed) complementary constraints \cite{Kim2023ContactImplicitMC, Cleach2021FastCM}, smooth surrogate models \cite{Pang2022GlobalPF, nol2018ContactImplicitTO}, or direct sampling of control \cite{Howell2022PredictiveSR}.
%
Aydinoglu et al. \cite{Aydinoglu2023ConsensusCC} proposed an operator splitting framework to decouple variables across time steps, and accelerated the intractable Linear Complementary Problem (LCP) for efficient manipulation.
%
Smoothing is discovered as an important procedure to enable exploration among contact modes and avoid falling into local minimum \cite{Kim2023ContactImplicitMC, Cleach2021FastCM}. Pang et al. \cite{Pang2022GlobalPF} proved that both randomized and analytic smoothing play a crucial part in dexterous manipulation planning.
%
Another method to obtain smooth dynamics is through compliant contact models \cite{nol2018ContactImplicitTO}. Inspired by Hunt and Crossley model, Kurtz et al. \cite{Kurtz2023InverseDT} proposed an alternative version with regularized friction, and passed the gradients through inverse dynamics. Although their method works well in the dexterous manipulation domain, the performance is easily affected by model parameters.
%
Despite the fact that contact-implicit methods improve efficiency by getting rid of dependence on specific contact sequences, the smoothing procedure produces the force-at-a-distance side effect \cite{Pang2022GlobalPF}. Thus, these methods often fail under even mild discrepancy between actual and planned contact modes.
%
In contrast, our method is more robust with contact feedback.
%


==> chapters/3_background.tex <==
%
This paper considers the quasi-static manipulation through rigid frictional contacts \cite{Mason2001MechanicsOR}. The object being manipulated is modelled as a single rigid body, while the manipulator can be any multi-link system, e.g., a multi-finger hand. Note that the manipulator makes contacts using any rigid part without specific end-effectors. The task is defined as moving the object from arbitrary start pose to desired pose.
%

%
‘Quasi-static’ refers to the inertia effects being negligible, in which the system has slow motion and can be described with first-order dynamics \cite{Jiang2023ContactAwareNM}. We make such an assumption because 1) it makes the system more suitable for precise manipulation, 2) it accords with many objects of daily life due to frictional surfaces, damped hinges or slow motions. In this paper, we use subscripts $o$, $r$ for object and robot, and $\Vert \cdot \Vert_{\bm{W}}$ for weighted norm unless otherwise stated. Besides, $\left[\bm{a}; \bm{b}\right]$ denotes the vertical concatenation of vectors $\bm{a}, \bm{b}$, $\left[\bm{A};\bm{B}\right]$ denotes the vertical stacking of matrices $\bm{A}, \bm{B}$.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_framework.pdf}
    \vspace{-15pt}
    \caption{\textbf{Block diagram of the proposed method.} The long-horizon contact-rich manipulation is accomplished by the contact reference generator and the contact controller working as a hierarchical structure.}
    \label{fig: block_diagram_proposed_method}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contact-Implicit Reference Generator}
\label{sec: reference_generator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
One key issue to achieve long-horizon in-hand manipulation is to auto-generate contact references online, i.e., hand configurations, reaction forces and so on for the low-level controller. The process accepts only desired object motion as input without any pre-defined sequences or trajectories.
%

%
\subsubsection{Problem Formulation}\label{sec: high_level_problem_formulation}
%
The generation of references is describes as an finite horizon optimal control problem.
\begin{equation}
    \begin{aligned}
        \min_{\bm{U}=\{\bm{u}_0,\cdots,\bm{u}_{N-1}\}} \quad & \sum_{i=0}^{N-1}l(\bm{x}_i,\bm{u}_i)+l_f(\bm{x}_N)\\
        \mbox{s.t.}\quad
        &\bm{x}_{i+1}=\bm{f}(\bm{x}_i,\bm{u}_i)\\
        & \underline{\bm{u}} \preceq \bm{u}_i \preceq \overline{\bm{u}},\ i=0,\dots,N-1 \\
    \end{aligned}
    \label{eq: high_level_oc_problem}
\end{equation}
For quasi-static manipulation, the state variables only include generalized positions, $\bm{x}=\bm{q}$. Besides, control inputs are chosen as $\bm{u}=\bm{S}_r\delta\bm{q}$ with the same bounds $\underline{\bm{u}},\overline{\bm{u}}$ at different time steps, where $\bm{S}_r$ selects the actuated dimensions. We expect the dynamics $\bm{f}$ to 1) evaluate efficiently, 2) have smooth forward and backward pass, 3) satisfy quasi-static assumptions. Property 2) is indicated in \cite{Kim2023ContactImplicitMC}, where smoothed gradients enable efficient transition among different contact modes. Moreover, we illustrate that unlike the exact integration as in \cite{Kim2023ContactImplicitMC}, the smooth forward pass is also indispensable for contact-implicit optimization in manipulation domain.
%

%
\subsubsection{Differentiable Dynamics Through Contact}\label{sec: high_level_dynamics}
%
For the dynamics mapping $\bm{f}$, we use the convex, quasi-dynamic, differentiable contact (CQDC) model \cite{Pang2022GlobalPF}, which has the above-mentioned properties. The model is exactly an optimization-based dynamics which relaxes the nonlinear contact mechanism as Cone Complementary Problem (CCP) \cite{Lidec2023ContactMI}:
\begin{equation}
    \begin{aligned}
        \min_{\bm{v}} \quad & \frac{1}{2}\bm{v}^\top\bm{Q}\bm{v}+\bm{b}^\top\bm{v} \\
        \mbox{s.t.}\quad
        & \mu_i\Vert \bm{J}_{i,t}\bm{v} \Vert_2 \leq \bm{J}_{i,n}\bm{v}+\phi_i,\ i=1,\dots,N_c \\
    \end{aligned},
    \label{eq: high_level_differentiable_dynamics}
\end{equation}
where $\phi_i, \mu_i$ are the signed distance, friction coefficient of the $i^{\text{th}}$ contact, and $\bm{J}=\left[\bm{J}_{i,n};\bm{J}_{i,t}\right]$ is the contact Jacobian. Besides, $\bm{Q}\triangleq\left[\bm{M}_o/h^2,\ 0;\ 0,\ \bm{K}_r\right]$, and $\bm{b}\triangleq-\left[\bm{\tau}_o;\ \bm{K}_r\bm{u}+\bm{\tau}_r\right]$, where $\bm{M}_o$ is the inertia matrix, $\bm{K}_r$ is the joint impedance, $\bm{\tau}_o,\bm{\tau}_r$ are generalized torques, and $h$ is the discrete time step. As described in \cite{Boyd_Vandenberghe_2011}, such a Second-Order Cone Programming (SOCP) can be solved with barrier method. We can choose the logarithm barrier function
\begin{equation}
    \zeta(\bm{v})=-\sum_{i=1}^{N_c}\log\left(\left(\bm{J}_{i,n}\bm{v}+\phi_i\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v} \Vert_2^2\right)
\end{equation}
Once the penalized problem is solved with parameter $\kappa>0$, we obtain the generalized velocities as primal solutions $\bm{v}^{*}(\kappa)$ and reaction forces as dual solutions
\begin{equation}
    \bm{\lambda}_i^{*}(\kappa)=\frac{2}{\kappa\alpha_i}
    \left[
        \begin{aligned}
            &\bm{J}_{i,n}\bm{v}^{*}+\phi_i \\
            &-\mu_i\bm{J}_{i,t}\bm{v}^{*}
        \end{aligned}
    \right],\ i=1,\dots,N_c
\end{equation}
where $\alpha_i=\left(\bm{J}_{i,n}\bm{v}^{*}+\phi_i\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v}^{*} \Vert_2^2$.
% KKT conditions of the unconstrained problem can be written as
% \begin{equation}
%     \bm{g}=\bm{Q}\bm{v}^{*}+\bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{\top})=\bm{0}
%     \label{eq: KKT_condition_compliant_model}
% \end{equation}
% where $\bm{Q}, \bm{b}$ is constant w.r.t $\bm{v}$, and $\bm{Q}$ is constant w.r.t. $\bm{q}$.
Then the smoothed gradients can be extracted as
\begin{equation}
    \frac{\partial \bm{v}^{*}}{\partial \bm{\xi}}=-\bm{H}^{-1}\frac{\partial}{\partial \bm{\xi}}\left(\bm{g}-\bm{Q}\bm{v}^{*}\right),\ \xi=\bm{q},\bm{u}
    \label{eq: gradient of SOCP}
\end{equation}
where
\begin{equation}
    \begin{aligned}
        \bm{g}-\bm{Q}\bm{v}^{*} &= \bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{*}) \\
        \bm{H} &= \bm{Q}+\frac{1}{\kappa}\nabla^2\zeta(\bm{v}^{*})
    \end{aligned}
\end{equation}
The gradients can be efficiently computed with kinematic Jacobians and Hessians from Pinocchio library \cite{carpentier2019pinocchio}. We can then obtain the differential terms $\bm{f}_{\bm{x}}, \bm{f}_{\bm{u}}$ given (\ref{eq: gradient of SOCP}).
%

%
\subsubsection{Cost Function Design}\label{sec: high_level_cost_function}
%
The cost functions is composed of three parts
\begin{equation}
    \begin{aligned}
        l(\bm{x},\bm{u}) &= C_o(\bm{x})+C_r(\bm{x})+C_u(\bm{u}) \\
        l_f(\bm{x}_N) &= C_o(\bm{x}_N)+C_r(\bm{x}_N)
    \end{aligned},
    \label{eq: high_level_differentiable_costs}
\end{equation}
%
the subscripts are omitted for brevity. The regulation costs
\begin{equation}
    \begin{aligned}
        C_o(\bm{x}) &= \Vert \bm{q}_o-\bm{q}_{o,\text{ref}} \Vert_{\bm{W}_o}^2 \\
        C_r(\bm{x}) &= \Vert \bm{q}_r-\bm{q}_{r,\text{ref}} \Vert_{\bm{W}_r}^2
    \end{aligned}
    \label{eq: high_level_regulation_costs}
\end{equation}
are the keys to generate contact-rich motions, where $\bm{q}_{\cdot,\text{ref}}$ are references and $\bm{W}_{\cdot}$ are weight matrices. Among them, $C_o$ guarantees desired object motions, and $C_r$ resets the fingers periodically to enable long-horizon manipulation. The negligence of $C_r$ often causes the system to fall into local optimum, i.e., the hand fails to actively break contacts. In practice, we find it helpful to increase $W_r$ near end of the receding horizon.
%

%
We also find that the consideration of control regulation terms improves numerical conditions and accelerates convergence.
\begin{equation}
    C_u(\bm{u}) = \Vert \bm{u} \Vert_{\bm{W}_u}^2
\end{equation}
%

%
Note that the framework is amenable to other types of costs, as long as they are differentiable. For example, additional costs can be introduced to encourage symmetric motions of certain fingers, and to enhance contact clearance or maintenance.
%

\subsubsection{Generation of Contact References}\label{sec: high_level_contact_reference_generation}
%
With differentiable dynamics (\ref{eq: high_level_differentiable_dynamics}) and costs (\ref{eq: high_level_differentiable_costs}), the optimal control problem (\ref{eq: high_level_oc_problem}) can be efficiently solved with the control-limited version of DDP \cite{Tassa2014ControllimitedDD}. We implement the algorithm using Python bindings of the Crocoddyl library \cite{mastalli20crocoddyl}. As suggested by \cite{Kim2023ContactImplicitMC}, we omit the second order terms $\bm{f}_{\bm{xx}}, \bm{f}_{\bm{ux}}, \bm{f}_{\bm{uu}}$ since they contain derivatives with higher orders than kinematic Hessian, and have weaker effects on convergence. In addition, we use larger regulation terms for state and control variables, which greatly promotes the convergence.
%

%
Finally, the solved trajectories $\bm{X}^{*}=\{\bm{x}_0^{*},\cdots\bm{x}_N^{*}\}, \bm{U}^{*}=\{\bm{u}_0^{*},\cdots\bm{u}_{N-1}^{*}\}, \bm{\Lambda}^{*}=\{\bm{\lambda}_1^{*},\cdots,\bm{\lambda}_{N-1}^{*}\}$ are converted to desired robot configurations and contact forces and interpolated before being sent to low-level controller.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_grasping.pdf}
    \vspace{-15pt}
    \caption{\textbf{Modeling of the contact controller.} The frames $\bm{O}_r,\bm{O}_c,\bm{O}_d$, frame displacements $d\bm{p}_{c,r},d\bm{p}_{r,d},d\bm{p}_o$, contact jacobians $\bm{G}_i,\bm{J}_i$, stiffness  matrices $\bm{K}_c,\bm{K}_r,\bm{K}_o$, and reaction force $\bm{F}_e$ are illustrated. Note that $\bm{O}_d$ can be obtained with forward kinematics $\bm{FK}(\bm{q}_d)$. The model compliance creates a coupling effect between force and motion.}
    \label{fig: grasping_annotations}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Compliance-Based Contact Controller}
\label{sec: contact_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
To mitigate the modeling errors originated from smooth contact models, we proposed a model-based controller to locally adjust the generated references. The controller incorporates an equivalent spring-damper system with the compliant contact model proposed in \cite{Kurtz2023InverseDT}. By coupling joint positions and reaction forces with compliance, a balance is achieved in tracking both factors.
%

%
\subsubsection{Compliant Contact Model}\label{sec: low_level_compliant_model}
%
The compliant model maps relative contact positions and velocities to reaction forces.
\begin{equation}
    \begin{aligned}
        f_n(\phi,\dot{\phi}) &= \sigma k \log\left(1+e^{-\frac{\phi}{\sigma}}\right)d_n(\dot{\phi})
        % \\
        % f_t(\phi, \dot{\phi}, \dot{\psi}) &= -\mu\frac{\dot{\psi}}{\sqrt{v_s^2+\dot{\psi}^2}}f_n(\phi,\dot{\phi})
    \end{aligned},
    \label{eq: parameterized_compliant_contact_model}
\end{equation}
where the dissipation factor $d_n(\dot{\phi})=\left(1-\dot{\phi}/v_d\right)\mathbb{I}_{\{\dot{\phi}<0\}}+0.25(\dot{\phi}/v_d-2)^2\mathbb{I}_{\{0\leq\dot{\phi}<2v_d\}}$, 
% $\dot{\phi},\dot{\psi}$ are normal and tangential contact velocities, and $\sigma, k, v_s, v_d$ are hyper-parameters.
$\dot{\phi}$ is the normal contact velocities, and $\sigma, k, v_d$ are hyper-parameters.
The compliant contact model is guaranteed to have continuous gradients. Thus we can define the spring-damper system in the contact frame,
\begin{equation}
    ^{C}\bm{K}_c=
    \begin{bmatrix}
	 0 & 0 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & \frac{\partial f_n}{\partial \phi}
    \end{bmatrix}
  %   ,
  %   ^{C}\bm{D}_c=
  %   \begin{bmatrix}
	 % 0 & 0 & 0 \\
  %     0 & \frac{\partial f_t}{\partial \dot{\psi}} & \frac{\partial f_t}{\partial \dot{\phi}}\\
  %     0 & 0 & \frac{\partial f_n}{\partial \dot{\phi}}
  %   \end{bmatrix}
  \label{eq: contact_stiffness_matrix}
\end{equation}
where y-axis aligns with the sliding direction, and z-axis coincides with the contact normal.
%

%-----------------------------------------------%
% For the subsection, we provide two versions
% One assume the contact positions remain unchanged
% while the other does not make such an assumption.
%-----------------------------------------------%
% ~~~~~~~~~~ The first version ~~~~~~~~~~ %
% %
% \subsubsection{Contact Force-Motion Model (A)}\label{sec: contact_force_motion_model}
% %
% We make the following assumptions: 1) the contact positions remain unchanged over the prediction horizon, 2) the contact stiffness and jacobian matrices are evaluated only once at the beginning.
% %
% Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
% %

% %
% The reaction force can be written as
% \begin{equation}
%     \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}+\bm{D}_{c}\dot{\bm{p}}_r
%     \label{eq: spring_damper_external_force}
% \end{equation}
% where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}, \bm{D}_c=\bm{R}_{C}\lvert^{C}\bm{D}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the frame displacement and $\dot{\bm{p}}_r$ is the contact velocity. As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
% \begin{equation}
%     \bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\bm{\dot{q}})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
%     \label{eq: pd_controller_result_force_balance}
% \end{equation}
% where $\bm{\mathcal{J}}=\left[\bm{J}_1,\cdots,\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1,\cdots,\bm{F}_{N_c}\right]$.
% Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}, \bm{J}(\dot{\bm{q}}_d-\bm{\dot{q}})=d\dot{\bm{p}}_{r,d}$, we can obtain that
% \begin{equation}
%     k_{p}d\bm{p}_{r,d}+k_{d}d\dot{\bm{p}}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
%     \label{eq: joint_impedance_external_force}
% \end{equation}
% Inspired from \cite{Gold2023ModelPI}, if we use
% \begin{equation}
%     d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
% \end{equation}
% and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
% \begin{equation}
%     \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=k_d\bm{K}_{c}\dot{\bm{p}}_d+\bm{K}_{c}d\bm{p}_{c,d}+\left(\bm{D}_{c}-k_d\bm{K}_{c}\right)\dot{\bm{p}}_r
%     \label{eq: mapping_from_motion_to_contact_force}
% \end{equation}
% Collecting (\ref{eq: mapping_from_motion_to_contact_force}) for all contacts and differentiating it with respect to time, we can obtain that
% % \begin{equation}
% %     \dot{\bm{F}}_e 
% % \approx \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\ddot{\bm{q}}_d+\dot{\bm{q}}_d\right)
% %     \label{eq: derivative_of_fe}
% % \end{equation}
% \begin{equation}
%     \dot{\bm{\mathcal{F}}}_e 
% \approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
%     \label{eq: derivative_of_fe}
% \end{equation}
% where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$.
% % The second-order term $\ddot{\bm{p}}_r$ is omitted under quasi-static assumption.
% The second-order terms $\ddot{\bm{q}}_d, \ddot{\bm{p}}_r$ are omitted under quasi-static assumption.
% From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
% \begin{equation}
%     \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
%     \label{eq: derivative_of_q}
% \end{equation}
% With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
% % \begin{equation}
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}} \\
% %       \dot{\bm{q}}_d \\
% %       \ddot{\bm{q}}_d \\
% %       \dot{\bm{F}}_e
% %     \end{bmatrix}
% %     \triangleq
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{J}^{\top}\bm{F}_e\right) \\
% %       \dot{\bm{q}}_d \\
% %       \tilde{\bm{u}} \\
% %       \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\tilde{\bm{u}}+\dot{\bm{q}}_d\right)
% %     \end{bmatrix}
% % \end{equation}
% \begin{equation}
%     \begin{bmatrix}
% 	 \dot{\bm{q}} \\
%       \dot{\bm{q}}_d \\
%       \dot{\bm{\mathcal{F}}}_e
%     \end{bmatrix}
%     \triangleq
%     \begin{bmatrix}
% 	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
%       \tilde{\bm{u}} \\
%       \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
%     \end{bmatrix}
%     \label{eq: quasi_static_contact_dynamics}
% \end{equation}
% %
% Note that (\ref{eq: quasi_static_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
% \begin{align}
%     \min_{\bm{U}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
%     & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \bm{u}_i-\bar{\bm{u}}_i \Vert_{\bm{W}_u} \nonumber \\
%     \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
%     &\bm{x}_{i+1}=\bm{A}\bm{x}_i+\bm{B}\bm{u}_i,\ i=0,\dots,N-1
% \end{align}
% where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\bm{u}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
% %

% ~~~~~~~~~~ The second version ~~~~~~~~~~ %
%
\subsubsection{Contact Force-Motion Model (B)}\label{sec: contact_force_motion_model}
%
We make the following assumptions: 1) quasi-static manipulation, 2) the contact stiffness and jacobian matrices are evaluated only once at the beginning.
%
Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
%
We extend the formulation in \cite{Gold2023ModelPI} to multi-contact cases.
%

%
Under quasi-static assumptions, the reaction force at each contact can be written as
\begin{equation}
    \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}
    \label{eq: spring_damper_external_force}
\end{equation}
where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the displacement between nearest points on the object and robot.
%
We attach a virtual spring at each contact with the stiffness matrix (\ref{eq: contact_stiffness_matrix}), and the equivalent stiffness $\bm{K}_o \in \mathbb{R}^{6 \times 6}$ can be obtained as
\begin{equation}
    \bm{K}_o = \sum_{i=1}^{N_c}\bm{G}_i^{\top}\bm{K}_{c,i}\bm{G}_{i}
\end{equation}
where $\bm{G}_i \in \mathbb{R}^{3 \times 6}$ equals the jacobian matrix of the $i^{\text{th}}$ contact. The grasping matrix $\bm{\mathcal{G}} \in \mathbb{R}^{3N_c \times 6}$ is defined as
\begin{equation}
    \bm{\mathcal{G}} = \left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right]
\end{equation}
%

%
As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
\begin{equation}
    \bm{K}_r(\bm{q}_d-\bm{q})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
    \label{eq: pd_controller_result_force_balance}
\end{equation}
where $\bm{\mathcal{J}}=\left[\bm{J}_1,\cdots,\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1,\cdots,\bm{F}_{N_c}\right]$.
Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}$, we can obtain that
\begin{equation}
    k_{p}d\bm{p}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
    \label{eq: joint_impedance_external_force}
\end{equation}
If we use
\begin{equation}
    d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
\end{equation}
and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
\begin{equation}
    \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=\bm{K}_{c}d\bm{p}_{c,d}
    \label{eq: mapping_from_motion_to_contact_force}
\end{equation}
Note that
\begin{equation}
    \begin{aligned}
        d\dot{\bm{p}}_{c,d} &= \dot{\bm{p}}_d-\dot{\bm{p}}_c \\
        &= \bm{J}\dot{\bm{q}}_d-\bm{G}_i\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\dot{\bm{\mathcal{F}}}_e
    \end{aligned}
    \label{eq: equations_between_force_and_motion_time_derivatives}
\end{equation}
Collecting (\ref{eq: mapping_from_motion_to_contact_force}) and (\ref{eq: equations_between_force_and_motion_time_derivatives}) for all contacts and differentiating it with respect to time, we can obtain that
\begin{equation}
    \dot{\bm{\mathcal{F}}}_e 
\approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\bar{\bm{G}}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
    \label{eq: derivative_of_fe}
\end{equation}
where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$, and $\bar{\bm{G}}=\left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right] \in \mathbb{R}^{3N_c \times 6}$.
From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
\begin{equation}
    \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
    \label{eq: derivative_of_q}
\end{equation}
With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
\begin{equation}
    \begin{bmatrix}
	 \dot{\bm{q}} \\
      \dot{\bm{q}}_d \\
      \dot{\bm{\mathcal{F}}}_e
    \end{bmatrix}
    \triangleq
    \begin{bmatrix}
	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
      \tilde{\bm{u}} \\
      \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\bar{\bm{G}}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
    \end{bmatrix}
    \label{eq: quasi_static_contact_dynamics}
\end{equation}
%
Note that (\ref{eq: quasi_static_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
\begin{align}
    \min_{\bm{U}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
    & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \bm{u}_i-\bar{\bm{u}}_i \Vert_{\bm{W}_u} \nonumber \\
    \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
    &\tilde{\bm{x}}_{i+1}=\bm{A}\tilde{\bm{x}}_i+\bm{B}\tilde{\bm{u}}_i,\ i=0,\dots,N-1
\end{align}
where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\bm{u}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Joint-Level PD Controller}
\label{sec: joint_level_pd_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
We use the joint-level pd controller with gravity compensation to convert the joint references $\bm{q}_d,\dot{\bm{q}}_d$ to joint torques $\bm{\tau}$.
\begin{equation}
    \bm{\tau}=\bm{\tau}_g+\bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\dot{\bm{q}})+\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}
    \label{eq: joint_level_control_law}
\end{equation}
where $\bm{\tau}_g$ is the generalized gravity. In addition, we add the feed-forward torque term 
% $\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}$
used in baseline methods and neglect inertia and Coriolis effects under quasi-static assumption.
%


==> chapters/3_background_v2.tex <==
%
This paper considers the quasi-static manipulation through rigid frictional contacts \cite{Mason2001MechanicsOR}. The object being manipulated is modelled as a single rigid body, while the manipulator can be any multi-link system, e.g., a multi-finger hand. Note that the manipulator makes contacts using any rigid part without specific end-effectors. The task is defined as moving the object from arbitrary start pose to desired pose.
%

%
‘Quasi-static’ refers to the inertia effects being negligible, in which the system has slow motion and can be described with first-order dynamics \cite{Jiang2023ContactAwareNM}. We make such an assumption because 1) it makes the system more suitable for precise manipulation, 2) it accords with many objects of daily life due to frictional surfaces, damped hinges or slow motions. In this paper, we use subscripts $o$, $r$ for object and robot, and $\Vert \cdot \Vert_{\bm{W}}$ for weighted norm unless otherwise stated. Besides, $\left[\bm{a}; \bm{b}\right]$ denotes the vertical concatenation of vectors $\bm{a}, \bm{b}$, $\left[\bm{A};\bm{B}\right]$ denotes the vertical stacking of matrices $\bm{A}, \bm{B}$.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_framework.pdf}
    \vspace{-15pt}
    \caption{\textbf{Block diagram of the proposed method.} The long-horizon contact-rich manipulation is accomplished by the contact reference generator and the contact controller working as a hierarchical structure.}
    \label{fig: block_diagram_proposed_method}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contact-Implicit Reference Generator}
\label{sec: reference_generator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
One key issue to achieve long-horizon in-hand manipulation is to auto-generate contact references online, i.e., hand configurations, reaction forces and so on for the low-level controller. The process accepts only desired object motion as input without any pre-defined sequences or trajectories.
%

%
\subsubsection{Problem Formulation}\label{sec: high_level_problem_formulation}
%
The generation of references is describes as an finite horizon optimal control problem.
\begin{equation}
    \begin{aligned}
        \min_{\bm{U}=\{\bm{u}_0,\cdots,\bm{u}_{N-1}\}} \quad & \sum_{i=0}^{N-1}l(\bm{x}_i,\bm{u}_i)+l_f(\bm{x}_N)\\
        \mbox{s.t.}\quad
        &\bm{x}_{i+1}=\bm{f}(\bm{x}_i,\bm{u}_i)\\
        & \underline{\bm{u}} \preceq \bm{u}_i \preceq \overline{\bm{u}},\ i=0,\dots,N-1 \\
    \end{aligned}
    \label{eq: high_level_oc_problem}
\end{equation}
For quasi-static manipulation, the state variables only include generalized positions, $\bm{x}=\bm{q}$. Besides, control inputs are chosen as $\bm{u}=\bm{S}_r\delta\bm{q}$ with the same bounds $\underline{\bm{u}},\overline{\bm{u}}$ at different time steps, where $\bm{S}_r$ selects the actuated dimensions. We expect the dynamics $\bm{f}$ to 1) evaluate efficiently, 2) have smooth forward and backward pass, 3) satisfy quasi-static assumptions. Property 2) is indicated in \cite{Kim2023ContactImplicitMC}, where smoothed gradients enable efficient transition among different contact modes. Moreover, we illustrate that unlike the exact integration as in \cite{Kim2023ContactImplicitMC}, the smooth forward pass is also indispensable for contact-implicit optimization in manipulation domain.
%

%
\subsubsection{Differentiable Dynamics Through Contact}\label{sec: high_level_dynamics}
%
For the dynamics mapping $\bm{f}$, we use the convex, quasi-dynamic, differentiable contact (CQDC) model \cite{Pang2022GlobalPF}, which has the above-mentioned properties. The model is exactly an optimization-based dynamics which relaxes the nonlinear contact mechanism as Cone Complementary Problem (CCP) \cite{Lidec2023ContactMI}:
\begin{equation}
    \begin{aligned}
        \min_{\bm{v}} \quad & \frac{1}{2}\bm{v}^\top\bm{Q}\bm{v}+\bm{b}^\top\bm{v} \\
        \mbox{s.t.}\quad
        & \mu_i\Vert \bm{J}_{i,t}\bm{v} \Vert_2 \leq \bm{J}_{i,n}\bm{v}+\phi_i,\ i=1,\dots,N_c \\
    \end{aligned},
    \label{eq: high_level_differentiable_dynamics}
\end{equation}
where $\phi_i, \mu_i$ are the signed distance, friction coefficient of the $i^{\text{th}}$ contact, and $\bm{J}=\left[\bm{J}_{i,n};\bm{J}_{i,t}\right]$ is the contact Jacobian. Besides, $\bm{Q}\triangleq\left[\bm{M}_o/h^2,\ 0;\ 0,\ \bm{K}_r\right]$, and $\bm{b}\triangleq-\left[\bm{\tau}_o;\ \bm{K}_r\bm{u}+\bm{\tau}_r\right]$, where $\bm{M}_o$ is the inertia matrix, $\bm{K}_r$ is the joint impedance, $\bm{\tau}_o,\bm{\tau}_r$ are generalized torques, and $h$ is the discrete time step. As described in \cite{Boyd_Vandenberghe_2011}, such a Second-Order Cone Programming (SOCP) can be solved with barrier method. We can choose the logarithm barrier function
\begin{equation}
    \zeta(\bm{v})=-\sum_{i=1}^{N_c}\log\left(\left(\bm{J}_{i,n}\bm{v}+\phi_i\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v} \Vert_2^2\right)
\end{equation}
Once the penalized problem is solved with parameter $\kappa>0$, we obtain the generalized velocities as primal solutions $\bm{v}^{*}(\kappa)$ and reaction forces as dual solutions
\begin{equation}
    \bm{\lambda}_i^{*}(\kappa)=\frac{2}{\kappa\alpha_i}
    \left[
        \begin{aligned}
            &\bm{J}_{i,n}\bm{v}^{*}+\phi_i \\
            &-\mu_i\bm{J}_{i,t}\bm{v}^{*}
        \end{aligned}
    \right],\ i=1,\dots,N_c
\end{equation}
where $\alpha_i=\left(\bm{J}_{i,n}\bm{v}^{*}+\phi_i\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v}^{*} \Vert_2^2$.
% KKT conditions of the unconstrained problem can be written as
% \begin{equation}
%     \bm{g}=\bm{Q}\bm{v}^{*}+\bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{\top})=\bm{0}
%     \label{eq: KKT_condition_compliant_model}
% \end{equation}
% where $\bm{Q}, \bm{b}$ is constant w.r.t $\bm{v}$, and $\bm{Q}$ is constant w.r.t. $\bm{q}$.
Then the smoothed gradients can be extracted as
\begin{equation}
    \frac{\partial \bm{v}^{*}}{\partial \bm{\xi}}=-\bm{H}^{-1}\frac{\partial}{\partial \bm{\xi}}\left(\bm{g}-\bm{Q}\bm{v}^{*}\right),\ \xi=\bm{q},\bm{u}
    \label{eq: gradient of SOCP}
\end{equation}
where
\begin{equation}
    \begin{aligned}
        \bm{g}-\bm{Q}\bm{v}^{*} &= \bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{*}) \\
        \bm{H} &= \bm{Q}+\frac{1}{\kappa}\nabla^2\zeta(\bm{v}^{*})
    \end{aligned}
\end{equation}
The gradients can be efficiently computed with kinematic Jacobians and Hessians from Pinocchio library \cite{carpentier2019pinocchio}. We can then obtain the differential terms $\bm{f}_{\bm{x}}, \bm{f}_{\bm{u}}$ given (\ref{eq: gradient of SOCP}).
%

%
\subsubsection{Cost Function Design}\label{sec: high_level_cost_function}
%
The cost functions is composed of three parts
\begin{equation}
    \begin{aligned}
        l(\bm{x},\bm{u}) &= C_o(\bm{x})+C_r(\bm{x})+C_u(\bm{u}) \\
        l_f(\bm{x}_N) &= C_o(\bm{x}_N)+C_r(\bm{x}_N)
    \end{aligned},
    \label{eq: high_level_differentiable_costs}
\end{equation}
%
the subscripts are omitted for brevity. The regulation costs
\begin{equation}
    \begin{aligned}
        C_o(\bm{x}) &= \Vert \bm{q}_o-\bm{q}_{o,\text{ref}} \Vert_{\bm{W}_o}^2 \\
        C_r(\bm{x}) &= \Vert \bm{q}_r-\bm{q}_{r,\text{ref}} \Vert_{\bm{W}_r}^2
    \end{aligned}
    \label{eq: high_level_regulation_costs}
\end{equation}
are the keys to generate contact-rich motions, where $\bm{q}_{\cdot,\text{ref}}$ are references and $\bm{W}_{\cdot}$ are weight matrices. Among them, $C_o$ guarantees desired object motions, and $C_r$ resets the fingers periodically to enable long-horizon manipulation. The negligence of $C_r$ often causes the system to fall into local optimum, i.e., the hand fails to actively break contacts. In practice, we find it helpful to increase $W_r$ near end of the receding horizon.
%

%
We also find that the consideration of control regulation terms improves numerical conditions and accelerates convergence.
\begin{equation}
    C_u(\bm{u}) = \Vert \bm{u} \Vert_{\bm{W}_u}^2
\end{equation}
%

%
Note that the framework is amenable to other types of costs, as long as they are differentiable. For example, additional costs can be introduced to encourage symmetric motions of certain fingers, and to enhance contact clearance or maintenance.
%

\subsubsection{Generation of Contact References}\label{sec: high_level_contact_reference_generation}
%
With differentiable dynamics (\ref{eq: high_level_differentiable_dynamics}) and costs (\ref{eq: high_level_differentiable_costs}), the optimal control problem (\ref{eq: high_level_oc_problem}) can be efficiently solved with the control-limited version of DDP \cite{Tassa2014ControllimitedDD}. We implement the algorithm using Python bindings of the Crocoddyl library \cite{mastalli20crocoddyl}. As suggested by \cite{Kim2023ContactImplicitMC}, we omit the second order terms $\bm{f}_{\bm{xx}}, \bm{f}_{\bm{ux}}, \bm{f}_{\bm{uu}}$ since they contain derivatives with higher orders than kinematic Hessian, and have weaker effects on convergence. In addition, we use larger regulation terms for state and control variables, which greatly promotes the convergence.
%

%
Finally, the solved trajectories $\bm{X}^{*}=\{\bm{x}_0^{*},\cdots\bm{x}_N^{*}\}, \bm{U}^{*}=\{\bm{u}_0^{*},\cdots\bm{u}_{N-1}^{*}\}, \bm{\Lambda}^{*}=\{\bm{\lambda}_1^{*},\cdots,\bm{\lambda}_{N-1}^{*}\}$ are converted to desired robot configurations and contact forces and interpolated before being sent to low-level controller.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_grasping.pdf}
    \vspace{-15pt}
    \caption{\textbf{Modeling of the contact controller.} The frames $\bm{O}_r,\bm{O}_c,\bm{O}_d$, frame displacements $d\bm{p}_{c,r},d\bm{p}_{r,d},d\bm{p}_o$, contact jacobians $\bm{G}_i,\bm{J}_i$, stiffness  matrices $\bm{K}_c,\bm{K}_r,\bm{K}_o$, and reaction force $\bm{F}_e$ are illustrated. Note that $\bm{O}_d$ can be obtained with forward kinematics $\bm{FK}(\bm{q}_d)$. The model compliance creates a coupling effect between force and motion.}
    \label{fig: grasping_annotations}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Compliance-Based Contact Controller}
\label{sec: contact_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
To mitigate the modeling errors originated from smooth contact models, we proposed a model-based controller to locally adjust the generated references. The controller incorporates an equivalent spring-damper system with the compliant contact model proposed in \cite{Kurtz2023InverseDT}. By coupling joint positions and reaction forces with compliance, a balance is achieved in tracking both factors.
%

%
\subsubsection{Compliant Contact Model}\label{sec: low_level_compliant_model}
%
The compliant model maps relative contact positions and velocities to reaction forces.
\begin{equation}
    \begin{aligned}
        f_n(\phi,\dot{\phi}) &= \sigma k \log\left(1+e^{-\frac{\phi}{\sigma}}\right)d_n(\dot{\phi})
        % \\
        % f_t(\phi, \dot{\phi}, \dot{\psi}) &= -\mu\frac{\dot{\psi}}{\sqrt{v_s^2+\dot{\psi}^2}}f_n(\phi,\dot{\phi})
    \end{aligned},
    \label{eq: parameterized_compliant_contact_model}
\end{equation}
where the dissipation factor $d_n(\dot{\phi})=\left(1-\dot{\phi}/v_d\right)\mathbb{I}_{\{\dot{\phi}<0\}}+0.25(\dot{\phi}/v_d-2)^2\mathbb{I}_{\{0\leq\dot{\phi}<2v_d\}}$, 
% $\dot{\phi},\dot{\psi}$ are normal and tangential contact velocities, and $\sigma, k, v_s, v_d$ are hyper-parameters.
$\dot{\phi}$ is the normal contact velocities, and $\sigma, k, v_d$ are hyper-parameters.
The compliant contact model is guaranteed to have continuous gradients. Thus we can define the spring-damper system in the contact frame,
\begin{equation}
    ^{C}\bm{K}_c=
    \begin{bmatrix}
	 0 & 0 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & \frac{\partial f_n}{\partial \phi}
    \end{bmatrix}
  %   ,
  %   ^{C}\bm{D}_c=
  %   \begin{bmatrix}
	 % 0 & 0 & 0 \\
  %     0 & \frac{\partial f_t}{\partial \dot{\psi}} & \frac{\partial f_t}{\partial \dot{\phi}}\\
  %     0 & 0 & \frac{\partial f_n}{\partial \dot{\phi}}
  %   \end{bmatrix}
  \label{eq: contact_stiffness_matrix}
\end{equation}
where y-axis aligns with the sliding direction, and z-axis coincides with the contact normal.
%

%-----------------------------------------------%
% For the subsection, we provide two versions
% One assume the contact positions remain unchanged
% while the other does not make such an assumption.
%-----------------------------------------------%
% ~~~~~~~~~~ The first version ~~~~~~~~~~ %
% %
% \subsubsection{Contact Force-Motion Model (A)}\label{sec: contact_force_motion_model}
% %
% We make the following assumptions: 1) the contact positions remain unchanged over the prediction horizon, 2) the contact stiffness and jacobian matrices are evaluated only once at the beginning.
% %
% Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
% %

% %
% The reaction force can be written as
% \begin{equation}
%     \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}+\bm{D}_{c}\dot{\bm{p}}_r
%     \label{eq: spring_damper_external_force}
% \end{equation}
% where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}, \bm{D}_c=\bm{R}_{C}\lvert^{C}\bm{D}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the frame displacement and $\dot{\bm{p}}_r$ is the contact velocity. As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
% \begin{equation}
%     \bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\bm{\dot{q}})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
%     \label{eq: pd_controller_result_force_balance}
% \end{equation}
% where $\bm{\mathcal{J}}=\left[\bm{J}_1,\cdots,\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1,\cdots,\bm{F}_{N_c}\right]$.
% Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}, \bm{J}(\dot{\bm{q}}_d-\bm{\dot{q}})=d\dot{\bm{p}}_{r,d}$, we can obtain that
% \begin{equation}
%     k_{p}d\bm{p}_{r,d}+k_{d}d\dot{\bm{p}}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
%     \label{eq: joint_impedance_external_force}
% \end{equation}
% Inspired from \cite{Gold2023ModelPI}, if we use
% \begin{equation}
%     d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
% \end{equation}
% and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
% \begin{equation}
%     \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=k_d\bm{K}_{c}\dot{\bm{p}}_d+\bm{K}_{c}d\bm{p}_{c,d}+\left(\bm{D}_{c}-k_d\bm{K}_{c}\right)\dot{\bm{p}}_r
%     \label{eq: mapping_from_motion_to_contact_force}
% \end{equation}
% Collecting (\ref{eq: mapping_from_motion_to_contact_force}) for all contacts and differentiating it with respect to time, we can obtain that
% % \begin{equation}
% %     \dot{\bm{F}}_e 
% % \approx \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\ddot{\bm{q}}_d+\dot{\bm{q}}_d\right)
% %     \label{eq: derivative_of_fe}
% % \end{equation}
% \begin{equation}
%     \dot{\bm{\mathcal{F}}}_e 
% \approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
%     \label{eq: derivative_of_fe}
% \end{equation}
% where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$.
% % The second-order term $\ddot{\bm{p}}_r$ is omitted under quasi-static assumption.
% The second-order terms $\ddot{\bm{q}}_d, \ddot{\bm{p}}_r$ are omitted under quasi-static assumption.
% From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
% \begin{equation}
%     \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
%     \label{eq: derivative_of_q}
% \end{equation}
% With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
% % \begin{equation}
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}} \\
% %       \dot{\bm{q}}_d \\
% %       \ddot{\bm{q}}_d \\
% %       \dot{\bm{F}}_e
% %     \end{bmatrix}
% %     \triangleq
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{J}^{\top}\bm{F}_e\right) \\
% %       \dot{\bm{q}}_d \\
% %       \tilde{\bm{u}} \\
% %       \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\tilde{\bm{u}}+\dot{\bm{q}}_d\right)
% %     \end{bmatrix}
% % \end{equation}
% \begin{equation}
%     \begin{bmatrix}
% 	 \dot{\bm{q}} \\
%       \dot{\bm{q}}_d \\
%       \dot{\bm{\mathcal{F}}}_e
%     \end{bmatrix}
%     \triangleq
%     \begin{bmatrix}
% 	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
%       \tilde{\bm{u}} \\
%       \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
%     \end{bmatrix}
%     \label{eq: quasi_static_contact_dynamics}
% \end{equation}
% %
% Note that (\ref{eq: quasi_static_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
% \begin{align}
%     \min_{\bm{U}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
%     & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \bm{u}_i-\bar{\bm{u}}_i \Vert_{\bm{W}_u} \nonumber \\
%     \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
%     &\bm{x}_{i+1}=\bm{A}\bm{x}_i+\bm{B}\bm{u}_i,\ i=0,\dots,N-1
% \end{align}
% where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\bm{u}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
% %

% ~~~~~~~~~~ The second version ~~~~~~~~~~ %
%
\subsubsection{Contact Force-Motion Model (B)}\label{sec: contact_force_motion_model}
%
We make the following assumptions: 1) quasi-static manipulation, 2) the contact stiffness and jacobian matrices are evaluated only once at the beginning.
%
Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
%
We extend the formulation in \cite{Gold2023ModelPI} to multi-contact cases.
%

%
Under quasi-static assumptions, the reaction force at each contact can be written as
\begin{equation}
    \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}
    \label{eq: spring_damper_external_force}
\end{equation}
where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the displacement between nearest points on the object and robot.
%
We attach a virtual spring at each contact with the stiffness matrix (\ref{eq: contact_stiffness_matrix}), and the equivalent stiffness $\bm{K}_o \in \mathbb{R}^{6 \times 6}$ can be obtained as
\begin{equation}
    \bm{K}_o = \sum_{i=1}^{N_c}\bm{G}_i^{\top}\bm{K}_{c,i}\bm{G}_{i}
\end{equation}
where $\bm{G}_i \in \mathbb{R}^{3 \times 6}$ equals the jacobian matrix of the $i^{\text{th}}$ contact. The grasping matrix $\bm{\mathcal{G}} \in \mathbb{R}^{3N_c \times 6}$ is defined as
\begin{equation}
    \bm{\mathcal{G}} = \left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right]
\end{equation}
%

%
As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
\begin{equation}
    \bm{K}_r(\bm{q}_d-\bm{q})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
    \label{eq: pd_controller_result_force_balance}
\end{equation}
where $\bm{\mathcal{J}}=\left[\bm{J}_1,\cdots,\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1,\cdots,\bm{F}_{N_c}\right]$.
Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}$, we can obtain that
\begin{equation}
    k_{p}d\bm{p}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
    \label{eq: joint_impedance_external_force}
\end{equation}
If we use
\begin{equation}
    d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
\end{equation}
and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
\begin{equation}
    \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=\bm{K}_{c}d\bm{p}_{c,d}
    \label{eq: mapping_from_motion_to_contact_force}
\end{equation}
Note that
\begin{equation}
    \begin{aligned}
        d\dot{\bm{p}}_{c,d} &= \dot{\bm{p}}_d-\dot{\bm{p}}_c \\
        &= \bm{J}\dot{\bm{q}}_d-\bm{G}_i\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\dot{\bm{\mathcal{F}}}_e
    \end{aligned}
    \label{eq: equations_between_force_and_motion_time_derivatives}
\end{equation}
Collecting (\ref{eq: mapping_from_motion_to_contact_force}) and (\ref{eq: equations_between_force_and_motion_time_derivatives}) for all contacts and differentiating it with respect to time, we can obtain that
\begin{equation}
    \dot{\bm{\mathcal{F}}}_e 
\approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\bar{\bm{G}}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
    \label{eq: derivative_of_fe}
\end{equation}
where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$, and $\bar{\bm{G}}=\left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right] \in \mathbb{R}^{3N_c \times 6}$.
From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
\begin{equation}
    \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
    \label{eq: derivative_of_q}
\end{equation}
With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
\begin{equation}
    \begin{bmatrix}
	 \dot{\bm{q}} \\
      \dot{\bm{q}}_d \\
      \dot{\bm{\mathcal{F}}}_e
    \end{bmatrix}
    \triangleq
    \begin{bmatrix}
	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
      \tilde{\bm{u}} \\
      \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\bar{\bm{G}}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
    \end{bmatrix}
    \label{eq: quasi_static_contact_dynamics}
\end{equation}
%
Note that (\ref{eq: quasi_static_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
\begin{align}
    \min_{\bm{U}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
    & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \bm{u}_i-\bar{\bm{u}}_i \Vert_{\bm{W}_u} \nonumber \\
    \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
    &\tilde{\bm{x}}_{i+1}=\bm{A}\tilde{\bm{x}}_i+\bm{B}\tilde{\bm{u}}_i,\ i=0,\dots,N-1
\end{align}
where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\bm{u}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Joint-Level PD Controller}
\label{sec: joint_level_pd_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
We use the joint-level pd controller with gravity compensation to convert the joint references $\bm{q}_d,\dot{\bm{q}}_d$ to joint torques $\bm{\tau}$.
\begin{equation}
    \bm{\tau}=\bm{\tau}_g+\bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\dot{\bm{q}})+\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}
    \label{eq: joint_level_control_law}
\end{equation}
where $\bm{\tau}_g$ is the generalized gravity. In addition, we add the feed-forward torque term 
% $\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}$
used in baseline methods and neglect inertia and Coriolis effects under quasi-static assumption.
%


==> chapters/4_method.tex <==
%
This paper considers the quasi-dynamic manipulation through rigid frictional contacts \cite{Mason2001MechanicsOR}. The object being manipulated is modelled as a single rigid body, while the manipulator can be any multi-link system, e.g., a multi-finger hand.
% Note that the manipulator makes contacts using any rigid part without specific end-effectors.
The task is defined as moving the object
% from arbitrary start pose to desired pose
to follow reference motions. The method is illustrated in Fig.~\ref{fig: block_diagram_proposed_method}.
%

%
‘Quasi-dynamic’ refers to the inertia effects being negligible, in which the momentum does not accumulate and the system can be described with first-order dynamics \cite{Pang2022GlobalPF, Jiang2023ContactAwareNM}. We make such an assumption because it accords with many objects of daily life due to frictional surfaces, damped hinges or slow motions. In this paper, we use subscripts $o$, $r$ for object and robot, and $\Vert \cdot \Vert_{\bm{W}}$ for weighted norm unless otherwise stated. Besides, $\left[\bm{a}; \bm{b}\right]$ denotes the vertical concatenation of vectors $\bm{a}, \bm{b}$, and $\left[\bm{A};\bm{B}\right]$ denotes the vertical stacking of matrices $\bm{A}, \bm{B}$.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_framework.pdf}
    \vspace{-15pt}
    \caption{\textbf{Block diagram of the proposed method.} The long-horizon contact-rich manipulation is accomplished by the contact reference generator and the contact controller working as a hierarchical structure.}
    \label{fig: block_diagram_proposed_method}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contact-Implicit Reference Generator}
\label{sec: reference_generator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
One key issue to achieve long-horizon in-hand manipulation is to auto-generate contact references online, i.e., hand configurations, reaction forces and so on for the low-level controller. The process accepts only desired object motion as input without any pre-defined sequences or trajectories.
%

%
\subsubsection{Problem Formulation}\label{sec: high_level_problem_formulation}
%
The generation of references is describes as an finite horizon optimal control problem.
\begin{equation}
    \begin{aligned}
        \min_{\bm{U}=\{\bm{u}_0,\cdots,\bm{u}_{N-1}\}} \quad & \sum_{i=0}^{N-1}l(\bm{x}_i,\bm{u}_i)+l_f(\bm{x}_N)\\
        \mbox{s.t.}\quad
        &\bm{x}_{i+1}=\bm{f}(\bm{x}_i,\bm{u}_i)\\
        & \underline{\bm{u}} \preceq \bm{u}_i \preceq \overline{\bm{u}},\ i=0,\dots,N-1 \\
    \end{aligned}
    \label{eq: high_level_oc_problem}
\end{equation}
For quasi-dynamic manipulation, the state variables only include generalized positions, i.e, $\bm{x}=\bm{q}$, with the dimension of $n_q$. Besides, control inputs are chosen as $\bm{u}=\bm{S}_r\delta\bm{q}$ with the same bounds $\underline{\bm{u}},\overline{\bm{u}}$ at different time steps, where $\bm{S}_r$ selects the actuated dimensions. We expect the dynamics $\bm{f}$ to 1) satisfy quasi-dynamic assumptions, 2) have smooth forward and backward passes, 3) evaluate efficiently. Property 2) is indicated in \cite{Kim2023ContactImplicitMC}, where smoothed gradients enable efficient transition among different contact modes. Moreover, we illustrate that unlike the exact integration as in \cite{Kim2023ContactImplicitMC}, the smooth forward pass is also indispensable for contact-implicit optimization in manipulation domain.
%

%
\subsubsection{Differentiable Dynamics Through Contact}\label{sec: high_level_dynamics}
%
For the dynamics mapping $\bm{f}$, we use the convex, quasi-dynamic, differentiable contact (CQDC) model \cite{Pang2022GlobalPF}, which has the above-mentioned properties. The model is exactly an optimization-based dynamics which relaxes the nonlinear contact mechanism as Cone Complementary Problem (CCP) \cite{Lidec2023ContactMI}:
\begin{equation}
    \begin{aligned}
        \min_{\bm{v}} \quad & \frac{1}{2}\bm{v}^\top\bm{Q}\bm{v}+\bm{b}^\top\bm{v} \\
        \mbox{s.t.}\quad
        & \mu_i\Vert \bm{J}_{i,t}\bm{v} \Vert_2 \leq \bm{J}_{i,n}\bm{v}+\phi_i/h,\ i=1,\dots,N_c \\
    \end{aligned},
    \label{eq: high_level_differentiable_dynamics}
\end{equation}
where $\bm{v}=\delta\bm{q}/h$, $\phi_i, \mu_i$ are the signed distance and friction coefficient of the $i^{\text{th}}$ contact, and $\bm{J}_i=\left[\bm{J}_{i,n};\bm{J}_{i,t}\right]$ is the contact Jacobian. Besides, $\bm{Q}\triangleq\left[\bm{M}_o/h,\ 0;\ 0,\ h\bm{K}_r\right]$, and $\bm{b}\triangleq-\left[\bm{\tau}_o;\ \bm{K}_r\bm{u}+\bm{\tau}_r\right]$, where $\bm{M}_o$ is the inertia matrix, $\bm{K}_r$ is the joint impedance, $\bm{\tau}_o,\bm{\tau}_r$ are generalized torques, and $h$ is the discrete time step. As described in \cite{Boyd_Vandenberghe_2011}, such a Second-Order Cone Programming (SOCP) can be solved with barrier method. We can choose the logarithm barrier function
\begin{equation}
    \zeta(\bm{v})=-\sum_{i=1}^{N_c}\log\left(\left(\bm{J}_{i,n}\bm{v}+\phi_i/h\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v} \Vert_2^2\right)
\end{equation}
Once the penalized problem is solved with parameter $\kappa>0$, we obtain the generalized velocities as primal solutions $\bm{v}^{*}(\kappa)$ and reaction forces as dual solutions
\begin{equation}
    \bm{\lambda}_i^{*}(\kappa)=\frac{2}{\kappa\alpha_i}
    \left[
        \begin{aligned}
            &\bm{J}_{i,n}\bm{v}^{*}+\phi_i/h \\
            &-\mu_i\bm{J}_{i,t}\bm{v}^{*}
        \end{aligned}
    \right],\ i=1,\dots,N_c
\end{equation}
where $\alpha_i=\left(\bm{J}_{i,n}\bm{v}^{*}+\phi_i/h\right)^2-\mu_i^2\Vert \bm{J}_{i,t}\bm{v}^{*} \Vert_2^2$.
% KKT conditions of the unconstrained problem can be written as
% \begin{equation}
%     \bm{g}=\bm{Q}\bm{v}^{*}+\bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{\top})=\bm{0}
%     \label{eq: KKT_condition_compliant_model}
% \end{equation}
% where $\bm{Q}, \bm{b}$ is constant w.r.t $\bm{v}$, and $\bm{Q}$ is constant w.r.t. $\bm{q}$.
Then the smoothed gradients can be extracted as
\begin{equation}
    \frac{\partial \bm{v}^{*}}{\partial \bm{\xi}}=-\bm{H}^{-1}\frac{\partial}{\partial \bm{\xi}}\left(\bm{g}-\bm{Q}\bm{v}^{*}\right),\ \xi=\bm{q},\bm{u}
    \label{eq: gradient of SOCP}
\end{equation}
where
\begin{equation}
    \begin{aligned}
        \bm{g}-\bm{Q}\bm{v}^{*} &= \bm{b}+\frac{1}{\kappa}\nabla\zeta(\bm{v}^{*}) \\
        \bm{H} &= \bm{Q}+\frac{1}{\kappa}\nabla^2\zeta(\bm{v}^{*})
    \end{aligned}
\end{equation}
The gradients can be efficiently computed with kinematic Jacobians and Hessians from Pinocchio library \cite{carpentier2019pinocchio}. We can then obtain the differential terms $\bm{f}_{\bm{x}}, \bm{f}_{\bm{u}}$ given (\ref{eq: gradient of SOCP}).
%

%
\subsubsection{Cost Function Design}\label{sec: high_level_cost_function}
%
The cost functions are composed of three parts
\begin{equation}
    \begin{aligned}
        l(\bm{x},\bm{u}) &= C_o(\bm{x})+C_r(\bm{x})+C_u(\bm{u}) \\
        l_f(\bm{x}_N) &= C_o(\bm{x}_N)+C_r(\bm{x}_N)
    \end{aligned},
    \label{eq: high_level_differentiable_costs}
\end{equation}
%
the subscripts are omitted for brevity. The regulation costs
\begin{equation}
    \begin{aligned}
        C_o(\bm{x}) &= \Vert \bm{q}_o-\bm{q}_{o,\text{ref}} \Vert_{\bm{W}_o}^2 \\
        C_r(\bm{x}) &= \Vert \bm{q}_r-\bm{q}_{r,\text{ref}} \Vert_{\bm{W}_r}^2
    \end{aligned}
    \label{eq: high_level_regulation_costs}
\end{equation}
are the keys to generate contact-rich motions, where $\bm{q}_{\cdot,\text{ref}}$ are references and $\bm{W}_{\cdot}$ are weight matrices. Among them, $C_o$ guarantees desired object motions, and $C_r$ resets the fingers periodically to enable long-horizon manipulation. The negligence of $C_r$ often causes the system to fall into local optimum, i.e., the hand fails to actively break contacts. In practice, we find it helpful to increase $W_r$ near end of the receding horizon.
%

%
We also find the consideration of control regulation terms improves numerical conditions and accelerates convergence.
\begin{equation}
    C_u(\bm{u}) = \Vert \bm{u} \Vert_{\bm{W}_u}^2
\end{equation}
%

%
Note that the framework allows other types of costs, as long as they are differentiable. For example, additional costs can be introduced to encourage symmetric motions of certain fingers, and to enhance contact clearance or maintenance.
%

\subsubsection{Generation of Contact References}\label{sec: high_level_contact_reference_generation}
%
With differentiable dynamics (\ref{eq: high_level_differentiable_dynamics}) and costs (\ref{eq: high_level_differentiable_costs}), the optimal control problem (\ref{eq: high_level_oc_problem}) can be efficiently solved with the control-limited version of DDP \cite{Tassa2014ControllimitedDD}.
% We implement the algorithm using Python bindings of the Crocoddyl library \cite{mastalli20crocoddyl}.
As suggested by \cite{Kim2023ContactImplicitMC}, we omit the second order terms $\bm{f}_{\bm{xx}}, \bm{f}_{\bm{ux}}, \bm{f}_{\bm{uu}}$ since they contain derivatives with higher orders than kinematic Hessian, and have weaker effects on convergence.
% In addition, we use larger regulation terms for state and control variables, which greatly promotes the convergence.
%

%
Finally, the solved trajectories $\bm{X}^{*}=\{\bm{x}_0^{*},\cdots\bm{x}_N^{*}\}, \bm{U}^{*}=\{\bm{u}_0^{*},\cdots\bm{u}_{N-1}^{*}\}, \bm{\Lambda}^{*}=\{\bm{\lambda}_1^{*},\cdots,\bm{\lambda}_{N-1}^{*}\}$ are converted to desired robot configurations and contact forces and interpolated before being sent to the low-level controller.
%

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs//method/method_grasping.pdf}
    \vspace{-15pt}
    \caption{\textbf{Modeling of the contact controller.} The frames $\bm{O}_r,\bm{O}_c,\bm{O}_d$, frame displacements $d\bm{p}_{c,r},d\bm{p}_{r,d},d\bm{p}_o$, contact jacobians $\bm{G}_i,\bm{J}_i$, stiffness  matrices $\bm{K}_c,\bm{K}_r,\bm{K}_o$, and reaction force $\bm{F}_e$ are illustrated. Note that $\bm{O}_d$ can be obtained with forward kinematics $\bm{FK}(\bm{q}_d)$. The model compliance creates a coupling effect between force and motion.}
    \label{fig: grasping_annotations}
    \vspace{-20pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Compliance-Based Contact Controller}
\label{sec: contact_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
To mitigate the modeling errors originated from smooth contact models, a model-based controller is proposed to locally adjust the generated references. The controller incorporates an equivalent mass-spring system with the compliant contact model proposed in \cite{Kurtz2023InverseDT}. By coupling joint positions and reaction forces with compliance, a balance is achieved in tracking both factors. The modeling is illustrated in Fig.~\ref{fig: grasping_annotations}.
%

%
\subsubsection{Compliant Contact Model}\label{sec: low_level_compliant_model}
%
The compliant model maps relative contact positions and velocities to reaction forces.
\begin{equation}
    \begin{aligned}
        f_n(\phi,\dot{\phi}) &= \sigma k \log\left(1+e^{-\frac{\phi}{\sigma}}\right)d_n(\dot{\phi})
        % \\
        % f_t(\phi, \dot{\phi}, \dot{\psi}) &= -\mu\frac{\dot{\psi}}{\sqrt{v_s^2+\dot{\psi}^2}}f_n(\phi,\dot{\phi})
    \end{aligned},
    \label{eq: parameterized_compliant_contact_model}
\end{equation}
where the dissipation factor $d_n(\dot{\phi})=\left(1-\dot{\phi}/v_d\right)\mathbb{I}_{\{\dot{\phi}<0\}}+0.25(\dot{\phi}/v_d-2)^2\mathbb{I}_{\{0\leq\dot{\phi}<2v_d\}}$, 
% $\dot{\phi},\dot{\psi}$ are normal and tangential contact velocities, and $\sigma, k, v_s, v_d$ are hyper-parameters.
$\dot{\phi}$ is the normal contact velocities, and $\sigma, k, v_d$ are hyper-parameters.
The compliant contact model is guaranteed to have continuous gradients. Thus we can define the equivalent stiffness in the contact frame,
\begin{equation}
    ^{C}\bm{K}_c=
    \begin{bmatrix}
	 0 & 0 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & \frac{\partial f_n}{\partial \phi}
    \end{bmatrix}
  %   ,
  %   ^{C}\bm{D}_c=
  %   \begin{bmatrix}
	 % 0 & 0 & 0 \\
  %     0 & \frac{\partial f_t}{\partial \dot{\psi}} & \frac{\partial f_t}{\partial \dot{\phi}}\\
  %     0 & 0 & \frac{\partial f_n}{\partial \dot{\phi}}
  %   \end{bmatrix}
  \label{eq: contact_stiffness_matrix}
\end{equation}
where y-axis aligns with the sliding direction, and z-axis coincides with the contact normal.
%

%-----------------------------------------------%
% For the subsection, we provide two versions
% One assume the contact positions remain unchanged
% while the other does not make such an assumption.
%-----------------------------------------------%
% ~~~~~~~~~~ The first version ~~~~~~~~~~ %
% %
% \subsubsection{Contact Force-Motion Model (A)}\label{sec: contact_force_motion_model}
% %
% We make the following assumptions: 1) the contact positions remain unchanged over the prediction horizon, 2) the contact stiffness and jacobian matrices are evaluated only once at the beginning.
% %
% Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
% %

% %
% The reaction force can be written as
% \begin{equation}
%     \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}+\bm{D}_{c}\dot{\bm{p}}_r
%     \label{eq: spring_damper_external_force}
% \end{equation}
% where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}, \bm{D}_c=\bm{R}_{C}\lvert^{C}\bm{D}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the frame displacement and $\dot{\bm{p}}_r$ is the contact velocity. As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
% \begin{equation}
%     \bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\bm{\dot{q}})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
%     \label{eq: pd_controller_result_force_balance}
% \end{equation}
% where $\bm{\mathcal{J}}=\left[\bm{J}_1,\cdots,\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1,\cdots,\bm{F}_{N_c}\right]$.
% Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}, \bm{J}(\dot{\bm{q}}_d-\bm{\dot{q}})=d\dot{\bm{p}}_{r,d}$, we can obtain that
% \begin{equation}
%     k_{p}d\bm{p}_{r,d}+k_{d}d\dot{\bm{p}}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
%     \label{eq: joint_impedance_external_force}
% \end{equation}
% Inspired from \cite{Gold2023ModelPI}, if we use
% \begin{equation}
%     d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
% \end{equation}
% and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
% \begin{equation}
%     \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=k_d\bm{K}_{c}\dot{\bm{p}}_d+\bm{K}_{c}d\bm{p}_{c,d}+\left(\bm{D}_{c}-k_d\bm{K}_{c}\right)\dot{\bm{p}}_r
%     \label{eq: mapping_from_motion_to_contact_force}
% \end{equation}
% Collecting (\ref{eq: mapping_from_motion_to_contact_force}) for all contacts and differentiating it with respect to time, we can obtain that
% % \begin{equation}
% %     \dot{\bm{F}}_e 
% % \approx \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\ddot{\bm{q}}_d+\dot{\bm{q}}_d\right)
% %     \label{eq: derivative_of_fe}
% % \end{equation}
% \begin{equation}
%     \dot{\bm{\mathcal{F}}}_e 
% \approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
%     \label{eq: derivative_of_fe}
% \end{equation}
% where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$.
% % The second-order term $\ddot{\bm{p}}_r$ is omitted under quasi-dynamic assumption.
% The second-order terms $\ddot{\bm{q}}_d, \ddot{\bm{p}}_r$ are omitted under quasi-dynamic assumption.
% From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
% \begin{equation}
%     \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
%     \label{eq: derivative_of_q}
% \end{equation}
% With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
% % \begin{equation}
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}} \\
% %       \dot{\bm{q}}_d \\
% %       \ddot{\bm{q}}_d \\
% %       \dot{\bm{F}}_e
% %     \end{bmatrix}
% %     \triangleq
% %     \begin{bmatrix}
% % 	 \dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{J}^{\top}\bm{F}_e\right) \\
% %       \dot{\bm{q}}_d \\
% %       \tilde{\bm{u}} \\
% %       \bar{\bm{K}}^{-1}\bm{K}_c\bm{J}\left(k_d\tilde{\bm{u}}+\dot{\bm{q}}_d\right)
% %     \end{bmatrix}
% % \end{equation}
% \begin{equation}
%     \begin{bmatrix}
% 	 \dot{\bm{q}} \\
%       \dot{\bm{q}}_d \\
%       \dot{\bm{\mathcal{F}}}_e
%     \end{bmatrix}
%     \triangleq
%     \begin{bmatrix}
% 	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
%       \tilde{\bm{u}} \\
%       \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
%     \end{bmatrix}
%     \label{eq: quasi_dynamic_contact_dynamics}
% \end{equation}
% %
% Note that (\ref{eq: quasi_dynamic_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
% \begin{align}
%     \min_{\bm{U}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
%     & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \bm{u}_i-\bar{\bm{u}}_i \Vert_{\bm{W}_u} \nonumber \\
%     \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
%     &\bm{x}_{i+1}=\bm{A}\bm{x}_i+\bm{B}\bm{u}_i,\ i=0,\dots,N-1
% \end{align}
% where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\bm{u}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
% %

% ~~~~~~~~~~ The second version ~~~~~~~~~~ %
%
% \subsubsection{Contact Force-Motion Model (B)}\label{sec: contact_force_motion_model}
\subsubsection{Contact Force-Motion Model}\label{sec: contact_force_motion_model}
%
We make the following assumptions: 1) quasi-dynamic manipulation, 2) the contact stiffness and Jacobian matrices are evaluated only once at the beginning of each control step.
%
Unless otherwise stated, we omit the subscript $i$, since the following derivation is the same for each contact.
%
We extend the formulation in \cite{Gold2023ModelPI} to multi-contact cases.
%

%
Under quasi-dynamic assumptions, the reaction force exerted by the robot at each contact can be written as
\begin{equation}
    \bm{F}_e=\bm{K}_{c} d\bm{p}_{c,r}
    \label{eq: spring_damper_external_force}
\end{equation}
where $\bm{K}_c=\bm{R}_{C}\lvert^{C}\bm{K}_c\rvert\bm{R}_{C}^{\top}$, $\bm{R}_C$ is the rotation matrix, and $\lvert\cdot\rvert$ is the element-wise absolute value operation. Besides, $d\bm{p}_{c,r}$ is the displacement between nearest points on the object and robot.
%
We attach a virtual spring at each contact with the stiffness matrix (\ref{eq: contact_stiffness_matrix}), and the equivalent stiffness $\bm{K}_o \in \mathbb{R}^{6 \times 6}$ can be obtained as
\begin{equation}
    \bm{K}_o = \sum_{i=1}^{N_c}\bm{G}_i^{\top}\bm{K}_{c,i}\bm{G}_{i}
\end{equation}
where $\bm{G}_i \in \mathbb{R}^{3 \times 6}$ equals the jacobian matrix of the $i^{\text{th}}$ contact. The grasping matrix $\bm{\mathcal{G}} \in \mathbb{R}^{3N_c \times 6}$ is defined as
\begin{equation}
    \bm{\mathcal{G}} = \left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right]
\end{equation}
%

%
% As described in Sec.~\ref{sec: joint_level_pd_controller}, the joint-level pd controller yields
According to (\ref{eq: joint_level_control_law}), the joint-level pd controller yields
\begin{equation}
    \bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\dot{\bm{q}})=\bm{\mathcal{J}}^\top(\bm{q})\bm{\mathcal{F}}_e
    \label{eq: pd_controller_result_force_balance}
\end{equation}
where $\bm{\mathcal{J}}=\left[\bm{J}_1;\cdots;\bm{J}_{N_c}\right]$, $\bm{\mathcal{F}}_e=\left[\bm{F}_1;\cdots;\bm{F}_{N_c}\right]$.
Typically we choose $\bm{K}_r=k_p\bm{I}, \bm{D}_r=k_d\bm{I}$ as diagonal matrices. Using $\bm{J}(\bm{q}_d-\bm{q}) \approx d\bm{p}_{r,d}$ and ignore the velocity term, we can obtain
\begin{equation}
    k_{p}d\bm{p}_{r,d}=\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e
    \label{eq: joint_impedance_external_force}
\end{equation}
If we use
\begin{equation}
    d\bm{p}_{c,d}=d\bm{p}_{c,r}+d\bm{p}_{r,d}
\end{equation}
and combines (\ref{eq: spring_damper_external_force}), (\ref{eq: joint_impedance_external_force}), we have
\begin{equation}
    \bm{F}_e+k_p^{-1}\bm{K}_c\bm{J}\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e=\bm{K}_{c}d\bm{p}_{c,d}
    \label{eq: mapping_from_motion_to_contact_force}
\end{equation}
Note that
\begin{equation}
    \begin{aligned}
        d\dot{\bm{p}}_{c,d} &= \dot{\bm{p}}_d-\dot{\bm{p}}_c \\
        &= \bm{J}\dot{\bm{q}}_d-\bm{G}_i\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\dot{\bm{\mathcal{F}}}_e
    \end{aligned}
    \label{eq: equations_between_force_and_motion_time_derivatives}
\end{equation}
Collecting (\ref{eq: mapping_from_motion_to_contact_force}) and (\ref{eq: equations_between_force_and_motion_time_derivatives}) for all contacts and differentiating it with respect to time, we can obtain that
\begin{equation}
    \dot{\bm{\mathcal{F}}}_e 
\approx \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\mathcal{G}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\dot{\bm{q}}_d
    \label{eq: derivative_of_fe}
\end{equation}
where $\bar{\bm{K}}=\left[\bm{K}_{c,1}\bm{J}_1;\cdots;\bm{K}_{c,N_c}\bm{J}_{N_c}\right] \in \mathbb{R}^{3N_c \times n_{q_r}}$. 
% and $\bar{\bm{G}}=\left[\bm{G}_1; \cdots; \bm{G}_{N_c}\right] \in \mathbb{R}^{3N_c \times 6}$
From (\ref{eq: pd_controller_result_force_balance}) it can be obtained that
\begin{equation}
    \dot{\bm{q}}=\dot{\bm{q}}_d+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right)
    \label{eq: derivative_of_q}
\end{equation}
With (\ref{eq: derivative_of_fe}) and (\ref{eq: derivative_of_q}), choosing the desired joint velocity as control input $\tilde{\bm{u}}=\dot{\bm{q}}_d$, and the second-order contact dynamics can be written as
\begin{equation}
    \begin{bmatrix}
	 \dot{\bm{q}} \\
      \dot{\bm{q}}_d \\
      \dot{\bm{\mathcal{F}}}_e
    \end{bmatrix}
    \triangleq
    \begin{bmatrix}
	 \tilde{\bm{u}}+k_d^{-1}\left(k_p(\bm{q}_d-\bm{q})-\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_e\right) \\
      \tilde{\bm{u}} \\
      \left(\bm{I}+k_p^{-1}\bar{\bm{K}}\bm{\mathcal{J}}^{\top}+\bar{\bm{G}}\bm{K}_o^{-1}\bm{\mathcal{G}}^{\top}\right)^{-1}\bar{\bm{K}}\tilde{\bm{u}}
    \end{bmatrix}
    \label{eq: quasi_dynamic_contact_dynamics}
\end{equation}
%
Note that (\ref{eq: quasi_dynamic_contact_dynamics}) describes the linear dynamics of $\Tilde{\bm{x}}=\left[\dot{\bm{q}}; \dot{\bm{q}}_d; \dot{\bm{\mathcal{F}}}_e\right]$. The low-level controller can be formulated as the following optimal control problem
\begin{align}
    \min_{\tilde{\bm{U}}} \  & \Vert \bm{q}_N-\bar{\bm{q}}_N \Vert_{\bm{W}_{q_{N}}} + \Vert \bm{\mathcal{F}}_{e,N}-\bar{\bm{\mathcal{F}}}_{e,N} \Vert_{\bm{W}_{F_N}} \nonumber \\
    & \sum_{i=0}^{N-1} \Vert \bm{q}_i-\bar{\bm{q}}_i \Vert_{\bm{W}_{x}} + \Vert \bm{\mathcal{F}}_{e,i}-\bar{\bm{\mathcal{F}}}_{e,i} \Vert_{\bm{W}_F} + \Vert \tilde{\bm{u}}_i-\bar{\tilde{\bm{u}}}_i \Vert_{\bm{W}_u} \nonumber \\
    \label{eq: low_level_oc_problem} \mbox{s.t.} \ 
    &\tilde{\bm{x}}_{i+1}=\bm{A}\tilde{\bm{x}}_i+\bm{B}\tilde{\bm{u}}_i,\ i=0,\dots,N-1
\end{align}
where the references $\bar{\bm{x}}_i,\bar{\bm{\mathcal{F}}}_{e,i},\bar{\tilde{\bm{u}}}_i$ are calculated from interpolating the generated references $\bm{X}^{*}, \bm{\Lambda}^{*}, \bm{U}^{*}$. The nominal joint references $\bm{q}_d,\dot{\bm{q}}_d$ are updated with $\tilde{\bm{u}}_0$.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Joint-Level PD Controller}
% \label{sec: joint_level_pd_controller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
We use the \textbf{joint-level pd controller} with gravity compensation to convert the joint references $\bm{q}_d,\dot{\bm{q}}_d$ to joint torques.
\begin{equation}
    \bm{\tau}=\bm{\tau}_g+\bm{K}_r(\bm{q}_d-\bm{q})+\bm{D}_r(\dot{\bm{q}}_d-\dot{\bm{q}})+\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}
    \label{eq: joint_level_control_law}
\end{equation}
where $\bm{\tau}_g$ is the generalized gravity. In addition, we add the feed-forward torque 
% $\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}$
used in baseline methods and neglect inertia and Coriolis effects under quasi-dynamic assumptions.
%


==> chapters/5_experiment.tex <==
%
We carry out simulations and ablation studies to validate the proposed method. The CQDC model is modified from the quasi-static simulator \cite{Pang2021ACQ} proposed by Pang et al. The DDP algorithm is implemented using Python bindings of the Crocoddyl library \cite{mastalli20crocoddyl}. Simulations of the complete system is conducted using Drake toolbox \cite{drake} and the codebase of \cite{Kurtz2023InverseDT} with hydroelastic contacts.
%

%
Two types of in-hand manipulation systems are used to evaluate the proposed method, as shown in Fig.~\ref{fig: test_cases}. We use a four-finger dexterous hand with fixed wrist and 16 actuated joints. The object being manipulated could either rotate perpendicular to the palm (\textbf{RotZ}, $n_q=17$) or be free-moving while being supported by the table (\textbf{Free}, $n_q=23$).
%

%
\begin{figure}[!t]
    \centering
    \subfigure[\textbf{RotZ}]{
        \begin{minipage}{4cm}
            \centering
            \includegraphics[width=4cm]{figs/experiments/test_case_1.png}
            \vspace{-0.2cm}
            \label{fig: rotz_system_testbench}
        \end{minipage}
    }
    \subfigure[\textbf{Free}]{
        \begin{minipage}{4cm}
            \centering    %子图居中
            \includegraphics[width=4cm]{figs/experiments/test_case_2.png}
            \vspace{-0.2cm}
            \label{fig: free_system_testbench}
        \end{minipage}
    }
    \vspace{-0.5cm}
    \caption{Two in-hand manipulation systems used in the experiments. The object being manipulated is painted in blue. (a) The orange cylinder represents a damped hinge. (b) The brown body represents the supporting plane.}
    \label{fig: test_cases}
    \vspace{-0.6cm}
\end{figure}
%

%
\begin{figure}[!b]
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=1\linewidth]{figs/experiments/kappa_change_v2.pdf}
    \vspace{-0.8cm}
    \caption{The relationship between $\kappa$ and optimization results. Cost of DDP, the object's yaw angle and the control input norms are plotted for 50 steps. Warmer colors indicate stronger smoothing effect.}
    \label{fig: kappa_change}
    % \vspace{-0.5cm}
\end{figure}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Long-Horizon Motion Generation with Rich Contacts} \label{sec: motion_generation_results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
We use $\kappa=100$ for all experiments throughout the paper, where a smaller value indicates stronger smoothing effect. We set the input bounds as $\SI{0.05}{rad}$ for the \textbf{RotZ} system and $\SI{0.2}{rad}$ for the \textbf{Free} system, with the discretization step $h=\SI{0.1}{s}$ and the horizon length of $\SI{10}{}$.
%

%
First, we demonstrate the importance of using smoothed forward dynamics for contact-rich manipulation. We command the object to rotate at $\SI{0.79}{rad/s}$ and change $\kappa$ in the computation of forward dynamics. As shown in Fig.~\ref{fig: kappa_change}, larger $\kappa$ leads to poorer convergence and less effective manipulation of the object. The yaw angles increase rapidly when $\kappa \geq \SI{1000}{}$, due to simultaneous finger motions solved from warm-start trajectories. However, they quickly evolve into vibrating motions or even stop moving after 20 iterations, without enough smoothing. Smoothed forward dynamics ($\kappa \leq 500$) enables the generation of finger-gaiting and achieves constant rotation speed, instead of getting stuck in a local optimum. Thus we prove it impossible to remedy high-level modeling errors through a more realistic forward pass. Hence a low-level controller is necessary.
%

%
Second, we test the generalization ability on different objects. As shown in Fig.~\ref{fig: teaser} and Fig.~\ref{fig: finger_gaiting}, a sphere with the radius of $\SI{6}{cm}$ and a cuboid with the side length of $\SI{7}{cm}$ are manipulated in the \textbf{RotZ} environment. The shaded areas indicate contact events ($\phi<\SI{3}{mm}$) of four fingers, where the finger-gaiting is auto-generated to accomplish the long-horizon manipulation. The sphere rotates at $\SI{0.29}{rad/s}$ and the cuboid rotates at $\SI{0.4}{rad/s}$. Our method seamlessly generalizes to different geometries
% even with non-differentiable contours
without any pre-training, which shows a potential advantage over learning-based approaches. See the attached video for details.
%

%
\begin{figure}[!t]
    \centering
    \subfigure[Cylinder]{
        \begin{minipage}{1\linewidth}
            \centering
            \includegraphics[height=2.5cm]{figs/experiments/cylinder_gait_v2.pdf}
            \hspace{-0.2cm}
            \includegraphics[height=2.5cm]{figs/experiments/cylinder_gait_shot.pdf}
        \end{minipage}
    }
    \subfigure[Cuboid]{
        \begin{minipage}{1\linewidth}
            \centering
            \vspace{-0.3cm}
            \includegraphics[height=2.5cm]{figs/experiments/cube_gait_v2.pdf}
            \hspace{-0.2cm}
            \includegraphics[height=2.5cm]{figs/experiments/cube_gait_shot.pdf}
        \end{minipage}
    }
    \vspace{-0.5cm}
    \caption{The finger-gaiting of the in-hand manipulation on two different objects, with the duration of 200 iterations. Shaded areas indicate contacts of each finger. The object yaw angle curves are plotted in grey.}
    \label{fig: finger_gaiting}
    \vspace{-0.6cm}
\end{figure}
%
%
\begin{figure}[!b]
    \vspace{-0.7cm}
    \centering
    \subfigure[Rotation]{
        \hspace{-0.3cm}
        \begin{minipage}{4.0cm}
            \centering
            \includegraphics[height=2.95cm]{figs/experiments/orientation_robustness_v2.pdf}
            \vspace{-0.4cm}
        \end{minipage}
    }
    \subfigure[Position]{
        \hspace{-0.2cm}
        \begin{minipage}{4.0cm}
            \centering    %子图居中
            \includegraphics[height=2.95cm]{figs/experiments/position_robustness_v2.pdf}
            \vspace{-0.4cm}
        \end{minipage}
    }
    \vspace{-0.2cm}
    \caption{The rotation and position error curves with the increasing amplitude of noise/disturbance. The mean values (solid lines) and half standard deviation ranges (shaded areas) are shown.}
    \label{fig: robustness_results}
    % \vspace{-0.6cm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version snapshots %
%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs//experiments//attachment/snapshots_valve.pdf}
%     \vspace{-0.2cm}
%     \caption{Snapshots of the long-horizon valve rotation task carried out in Drake simulator. The fingers perform side-pushes and step over the valve in succession. The valve is represented by the blue capsule, and rotates around the vertical axis. Red arrows represent the contact forces.}
%     \label{fig: valve_rotation_snapshots}
%     \vspace{-0.2cm}
% \end{figure*}
% %
%%%%%%%%%%%%%%%%%%%%%%%%%
% New version snapshots %
%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[!t]
    \centering
    \subfigure[Valve]{
        \begin{minipage}{1\linewidth}
            \centering
            \includegraphics[height=2.8cm]{figs/experiments/attachment/snapshots_valve_v3.pdf}
            \hspace{-0.5cm}
            \includegraphics[height=2.8cm]{figs/experiments/attachment/valve_progress_plot_v5.pdf}
            \vspace{-0.3cm}
            \label{fig: valve_rotation_snapshots}
        \end{minipage}
    }
    \subfigure[Sphere]{
        \begin{minipage}{1\linewidth}
            \centering
            \vspace{-0.32cm}
            \includegraphics[height=2.7cm]{figs/experiments/attachment/snapshots_sphere_v3.pdf}
            \includegraphics[height=2.8cm]{figs/experiments/attachment/sphere_rpy_error_plot_v5.pdf}
            \vspace{0.1cm}
            \label{fig: sphere_rotation_snapshots}
        \end{minipage}
    }
    \vspace{-0.5cm}
    \caption{Snapshots of the long-horizon (a) valve rotation task and (b) sphere rotation task carried out in Drake simulator. Red arrows represent the contact forces. (a) The valve is represented by the blue capsule, and rotates around the vertical axis. The fingers perform side-pushes and step over the valve in succession. (b) External disturbances are applied on the object and ring finger, as the white arrows indicate. Final state of the open-loop baseline is also shown. Object yaw angle and error curves are shown on the right.}
    \label{fig: snapshots_and_error_curves}
    \vspace{-0.25cm}
\end{figure*}
%

%
Third, we further evaluate the robustness of our method under external disturbances or internal noises, which are assumed to obey Gaussian distributions, with the standard deviation $\sigma$. The sphere is commanded to rotate around the vertical axis in the \textbf{Free} system. To simulate the disturbances, we apply numerical perturbations once to the Euler angles and change $\sigma$ (i.e., the magnitude) from $\SI{0.1}{rad}$ to $\SI{0.8}{rad}$. To simulate the noises, at every time step, we perturb the dimensions of hand, object position and quaternion in $\bm{x}$, with $\sigma=\SI{0.03}{rad},\SI{1}{mm},\SI{0.01}{}$, respectively. We define the amplitude as the multiples of $\sigma$. We run 100 random experiments for each parameter and record the average tracking error within 400 steps. As shown in Fig.~\ref{fig: robustness_results}, our method could recover from a wide range of disturbances and noises. Robustness is essential for long-horizon manipulation, under sensor noises, control delays and external disturbances. The orientation error explodes under large disturbances, since the system needs longer time for recovery.
%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robust Execution with Contact Controller}  \label{sec: contact_control_results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
\subsubsection{Simple tasks}  \label{sec: simple_tasks_low_level}
%
We choose three classes of baselines for comparison. The first class is executing generated trajectories in a open-loop fashion (Ours w/o ctrl), which resembles the motion planning in \cite{Pang2022GlobalPF} with online re-planning. The second class utilizes feed-forward torques $\bm{\tau}_{ff}=\bm{\mathcal{J}}^{\top}\bm{\mathcal{F}}_{e,ff}$ as (\ref{eq: joint_level_control_law}) (FF+torque), which is the quasi-dynamic variant of \cite{Kurtz2023InverseDT}. The third class maps feed-forward torques to desired positions, where $\bm{q}_d$ is replaced by $\bm{q}_d+\bm{\tau}_{ff}/\bm{K}_{\text{ctrl}}$ in (\ref{eq: joint_level_control_law}) (FF+pos), as suggested by \cite{Kim2023ContactImplicitMC}. 
%
As for our feedback design, low-cost tactile sensors \cite{Lambeta2020DIGITAN} can be used to obtain contact forces $\bm{\mathcal{F}}_{e}$ in hardware.
%
A slippage metric, 
% $L(\bm{q},\dot{\bm{q}})=\mathtt{Sigmoid}(c\phi)\Vert\bm{J}_{i,t}\bm{v}_t\Vert^2$
$L(\phi,\bm{v})=\mathtt{Sigmoid}(c\phi)\Vert\bm{J}_{i,t}\bm{v}\Vert^2$
, is adopted from \cite{Kim2023ContactImplicitMC} to indicate the occurrence of missed or ineffective contacts. We choose $c<0$ to penalize slippage when the finger is close to the object.
%

%
\begin{table}[!t]
    \centering
    \vspace{-0.3cm}
    \caption{Controller Performance in the RotZ System.}
    \vspace{-0.2cm}
    \label{tab: performace_low_level_ctrl}
        \begin{tabular}{@{}c|ccc@{}}
            \toprule
            Methods          & \begin{tabular}[c]{@{}c@{}c@{}}Average\\ slippage\\ ($\times 10^{-3}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}c@{}}Average\\ rotation speed\\ (rad/s)\end{tabular} & \begin{tabular}[c]{@{}c@{}c@{}}Average\\ joint velocity\\ (rad/s)\end{tabular} \\ \midrule
            Ours              & \textbf{3.26}   & 0.30  & 0.93     \\
            Ours w/o ctrl     & 8.04   & 0.05  & 0.83     \\
            FF+torque         & 9.47   & 0.85  & 1.17     \\
            FF+pos            & 8.80   & 0.85  & 1.18      \\ \bottomrule
        \end{tabular}
    \vspace{-0.6cm}
\end{table}
%

%
We simulate the \textbf{RotZ} system in Drake for $\SI{10.0}{s}$ with the four controllers. The reference generator outputs references at $\SI{20}{Hz}$ and the contact controller runs at $\SI{100}{Hz}$. We record the average slippage when $\phi<\SI{1}{mm}$, the object's average rotation speed and the hand's average speed in joint space.
%
As depicted in Table \ref{tab: performace_low_level_ctrl}, our controller achieves the lowest average slippage by maintaining enough desired force. As a result, the average rotation speed increases significantly compared with open-loop execution, which indicates more effective manipulation is achieved with our method. The two feed-forward controllers have similar performance, and rotates the sphere faster with higher slippage. This is because the feed-forward torques are converted into displacements due to joint impedance. Thus feed-forward controllers often result in larger deviation from planned motions, and faster joint velocities once the contact is lost, as seen in the last column of Table \ref{tab: performace_low_level_ctrl}. In contrast, our controller strikes a balance between tracking planned motions and making contacts, thus generating more stable motions.
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version errorcurves %
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \begin{figure}[!t]
%     \vspace{-0.3cm}
%     \centering
%     \subfigure[Valve]{
%         \begin{minipage}{1\linewidth}
%             \centering
%             \includegraphics[width=7cm]{figs/experiments/attachment/valve_progress_plot.pdf}
%             \label{fig: valve_yaw_plot}
%         \end{minipage}
%     }
%     \subfigure[Sphere]{
%         \hspace{-0.25cm}
%         \begin{minipage}{1\linewidth}
%             \centering
%             \vspace{-0.2cm}
%             \includegraphics[width=7.2cm]{figs/experiments/attachment/sphere_rpy_error_plot.pdf}
%             \label{fig: sphere_error_plot}
%         \end{minipage}
%     }
%     \vspace{-0.5cm}
%     \caption{(a) Object yaw angle curve in the valve rotation task. (b) Object orientation error curve in the sphere rotation task. Shaded areas show the time periods of external force disturbance.}
%     \label{fig: valve_and_sphere_error_plot}
%     \vspace{-0.8cm}
% \end{figure}
%

%
\subsubsection{Complex tasks}  \label{sec: complex_tasks_low_level}
%
We further evaluate the contact controller and the proposed method in more complex cases. These experiments also show potential applications in the real world. 
%

%
The first case is rotating the valve, where $n_q=17$. In this case, the fingers should switch between pushing aside and stepping over the valve to accomplish the long-horizon manipulation, shown in Fig.~\ref{fig: valve_rotation_snapshots}. To our best knowledge, such long-horizon manipulation is almost only studied in the machine-learning literature. We find it helpful to interpolate the joint reference $\bm{q}_{o,\text{ref}}$ between two configurations of different fingertip heights. Otherwise, longer horizon length is needed to avoid local optimums, which degrades control frequency. As shown in Fig.~\ref{fig: valve_rotation_snapshots}, the fingers sometimes need to exert forces below the valve, which is sensitive to contact loss. Our proposed contact controller effectively avoids such problems, as shown in the curves and the attached video.
%

%
The second case is rotating the sphere in place, where $n_q=19$. The sphere needs to be aligned with the target orientation in SO(3). With our proposed controller, we exert spatial force disturbances on the object during $\SI{2.0}{s}\sim\SI{2.5}{s}$ and on the ring finger during $\SI{10.0}{s}\sim\SI{10.5}{s}$.
% As shown in Fig.~\ref{fig: sphere_rotation_snapshots}, the disturbances lead to rapid increases in the orientation error, which soon converges with the proposed method.
% However, without the contact controller, the error decreases slowly mainly due to contact loss, and sometimes increases with unintentional contacts.
As shown in Fig.~\ref{fig: sphere_rotation_snapshots}, due to contact loss and unintentional contacts, the long-horizon manipulation fails without the contact controller.
Hence, the importance of our contact controller is proved.
%
We also simulate the \textbf{Free} system in Fig.~\ref{fig: free_system_testbench} and successfully rotate the sphere for more than $270^\circ$. However, the rolling contacts result in highly dynamic movements of the object, which violates the quasi-dynamic assumption and degrades the performance. We temporarily increase damping of the object. As suggested by \cite{Pang2022GlobalPF}, designing special high-level objectives and enforcing the system to be quasi-dynamic at low-level could help to solve this problem.
We leave them for future work.
%


==> chapters/6_conclusions.tex <==
%
This paper considers the task of long-horizon in-hand manipulation. First, the reference generator computes joint trajectories and reaction forces given only desired motions. Then, the contact controller with tactile feedback tracks joint motions and maintains the planned contacts in the presence of modeling errors. The experiments demonstrate that the proposed method achieves similar dexterity with learning-based approaches and generalizes to different objects without any pre-training. With the reference generator, our method accomplishes long-horizon manipulation without a separated planning procedure, by re-calculating the trajectories at real-time rates. With the contact controller, our method prevents contact loss and becomes more robust to disturbances. Future works will consider hardware implementation with tactile sensors, and improving the manipulation performance with hand-arm coordination.
%

